The importance of better models in stochastic optimization

Standard stochastic optimization methods are brittle, sensitive to stepsize choices and other algorithmic parameters, and they exhibit instability outside of well-behaved families of objectives. To address these challenges, we investigate models for stochastic minimization and learning problems that exhibit better robustness to problem families and algorithmic parameters. With appropriately accurate models---which we call the aProx family---stochastic methods can be made stable, provably convergent and asymptotically optimal; even modeling that the objective is nonnegative is sufficient for this stability. We extend these results beyond convexity to weakly convex objectives, which include compositions of convex losses with smooth functions common in modern machine learning applications. We highlight the importance of robustness and accurate modeling with a careful experimental evaluation of convergence time and algorithm sensitivity.

==> asymptotic-not-worse.tex <==
% -*- Mode: latex -*- %
\providecommand{\steppow}{\beta}

\section{Not Worse than SGM}
\label{sec:aProx-no-worse}
In this section, we show that using \emph{any} model of aProx cannot result with worse asymptotic convergence rates than SGM, both the in the convex and weakly convex cases. We start our analysis in the convex setting.


\subsection{Asymptotic convergence for weakly convex function}
Now, we give an asymptotic convergence guarantee for the weakly convex
case. In~\cite{DavisDr19, DavisGr17}, Davis et al. prove convergence guarantees for Lipschitz and weakly convex functions to a near stationary point; i.e. a point $x$ such that $\dist(0, \partial F(x)) \le \epsilon$. We prove similar convergence guarantees while replacing the Lipschitz requirement with the following weaker assumption.
\begin{assumption}
	\label{assumption:growth-subgrads}
	There exist constants $C_1 < \infty$ and $C_2 < \infty$
	such that for any measurable selection
	$f'(x;\statval) \in \partial f(x; \statval)$, we have
	$\E[\ltwo{f'(x;\statrv)}^2] \le C_1 F(x) + C_2$.
\end{assumption}
In the next convergence guarantees, we use the following
notation for the Moreau envelope and its minimizer.
For $x \in \R^n$, let
\begin{equation*}
x^\lambda \defeq \argmin_{y \in \mc{X}}
\left\{F(y) + \frac{\lambda}{2} \ltwo{y - x}^2
\right\},
\end{equation*}
and define the Moreau envelope function
\begin{equation*}
F_\lambda(x) \defeq \inf_{y \in \mc{X}}
\left\{F(y) + (\lambda/2) \ltwo{y - x}^2\right\}.
\end{equation*}
Similarly to~\cite{DavisDr19, DavisGr17}, we use the following properties of the Moreau envelope to prove convergence to near stationary point.
\begin{itemize}
	\item $\ltwo{x^\lambda  - x} = \lambda \ltwo{ \nabla F_\lambda(x) }$
	\item $F(x^\lambda) \le F(x)$
	\item $\dist(0; \nabla F(x^\lambda)) \le \ltwo{\nabla F_\lambda(x) }$
\end{itemize} 
Therefore, we deduce that a small value of $\ltwo{\nabla F_\lambda(x)}$, or similarly $\ltwo{x^\lambda  - x}$, implies that $x$ is near a point $x^\lambda$ that is nearly stationary.

In the following theorem, we present our main convergence result for the weakly convex case.
\begin{theorem}
	\label{theorem:as-convergence-weakly-convex}
	Let Conditions~\ref{cond:convex-model}--\ref{cond:subgrad-model}
	hold. Assume further that $F(x) \ge 0$ for all $x \in \mc{X}$.
	If $f(\cdot;\statval)$ is $\lipobj(\statval)$-Lipschitz,
	then
	\begin{equation}
	\label{eqn:weakly-convex-lipschitz-progress}
	\E[F_\lambda(x_{k+1}) \mid \mc{F}_{k-1}]
	\le F_\lambda(x_k)
	- \stepsize_k \frac{\lambda (\lambda - \wb{\weakconvexfunc})}{2}
	\ltwos{x_k - x_k^\lambda}^2
	+ \frac{\lambda \stepsize_k^2}{2} \E[\lipobj(\statrv)^2].
	\end{equation}
	If instead Assumption~\ref{assumption:growth-subgrads} holds,
	then for constants $A, B < \infty$, which may depend on $\lambda$,
	we have
	\begin{equation}
	\label{eqn:weakly-convex-nonlipschitz-progress}
	\E[F_\lambda(x_{k+1}) \mid \mc{F}_{k-1}]
	\le (1 + A \stepsize_k^2 ) F_\lambda(x_k)
	- \stepsize_k \frac{\lambda(\lambda - \wb{\weakconvexfunc})}{2}
	\ltwos{x_k - x_k^\lambda}^2
	+ \stepsize_k^2 B.
	\end{equation}
\end{theorem}







==> weakly-convex-convergence.tex <==
% -*- Mode: latex -*- %


\section{Asymptotic convergence}
\label{sec:convergence}
We begin our theoretical analysis by providing convergence guarantees for any model satisfying Conditions~\ref{cond:convex-model}--\ref{cond:subgrad-model}. Davis and colleagues~\cite{?} prove convergence to near stationary point when the functions $f$ are Lipschitz. Here, we consider a weaker requirement on the sub-gradients, that allows the gradients to be unbounded.
\begin{assumption}
	\label{assumption:growth-subgrads}
	There exist constants $C_1 < \infty$ and $C_2 < \infty$
	such that for any measurable selection
	$f'(x;\statval) \in \partial f(x; \statval)$, we have
	$\E[\ltwo{f'(x;\statrv)}^2] \le C_1 F(x) + C_2$.
\end{assumption}
Indeed, Assumption~\ref{assumption:growth-subgrads} is more general than Lipschitz, and holds in much broader range of problems; consider for example the quadratic functions $f(x; (a,b)) = (\<a,x\> - b)^2$ for linear regression and $f(x; (a,b)) = \left| \<a,x\>^2 - b \right|$ for phase retrieval. While these functions are not Lipschitz, it is easy to verify that Assumption~\ref{assumption:growth-subgrads} holds as long as $\E[\ltwo{a}^2] < \infty$. 
Throughout this section,
we without comment make the assumption that $F(x) \ge 0$ for $x \in \mc{X}$, and the stepsizes $\stepsize_k$
satisfy the standard summability conditions
\begin{equation*}
\stepsize_k > 0 ~ \mbox{for~all~} k,
~~~
\sum_{k=1}^\infty \stepsize_k = \infty,
~~~ \mbox{and} ~~~
\sum_{k=1}^\infty \stepsize_k^2 < \infty.
\end{equation*}

To provide our convergence guarantees, we first define the Moreau envelope and its minimizer. For $x \in \R^n$, let
\begin{equation*}
x^\lambda \defeq \argmin_{y \in \mc{X}}
\left\{F(y) + \frac{\lambda}{2} \ltwo{y - x}^2
\right\},
\end{equation*}
and define the Moreau envelope function
\begin{equation*}
F_\lambda(x) \defeq \inf_{y \in \mc{X}}
\left\{F(y) + \frac{\lambda}{2} \ltwo{y - x}^2\right\}.
\end{equation*}
Our convergence machinery, in similar to~\cite{DavisDr19, DavisGr17}, relies on the following properties of the Moreau envelope.
\begin{itemize}
	\item $\ltwo{x^\lambda  - x} = \lambda \ltwo{ \nabla F_\lambda(x) }$
	\item $F(x^\lambda) \le F(x)$
	\item $\dist(0; \nabla F(x^\lambda)) \le \ltwo{\nabla F_\lambda(x) }$
\end{itemize}
The goal, then, is to prove convergence to a point $x$ such that $\ltwo{x^\lambda  - x}$ is small, as this implies that $x$ is close to a nearly stationary point, that is $x^\lambda$.

The next lemma provides one step-progress guarantee for the iterates $x_k$, which will be used later to show convergence to a point that is close to nearly stationary point.
%We assume w.l.o.g. that $F(x) \ge 0$ for all $x \in \mc{X}$, since otherwise we can apply our analysis to $F_{+}(x) = F(x) - \inf_{y \in \mc{X}} F(y)$.
\begin{lemma}
  Let Conditions~\ref{cond:convex-model}--\ref{cond:subgrad-model}
  hold. 
  If $f(\cdot;\statval)$ is $\lipobj(\statval)$-Lipschitz,
  then
  \begin{equation}
    \label{eqn:weakly-convex-lipschitz-progress}
    \E[F_\lambda(x_{k+1}) \mid \mc{F}_{k-1}]
    \le F_\lambda(x_k)
    - \stepsize_k \frac{\lambda (\lambda - \wb{\weakconvexfunc})}{2}
    \ltwos{x_k - x_k^\lambda}^2
    + \frac{\lambda \stepsize_k^2}{2} \E[\lipobj(\statrv)^2].
  \end{equation}
  If instead Assumption~\ref{assumption:growth-subgrads} holds,
  then for constants $A, B < \infty$, which may depend on $\lambda$,
  we have
  \begin{equation}
    \label{eqn:weakly-convex-nonlipschitz-progress}
    \E[F_\lambda(x_{k+1}) \mid \mc{F}_{k-1}]
    \le (1 + A \stepsize_k^2 ) F_\lambda(x_k)
    - \stepsize_k \frac{\lambda(\lambda - \wb{\weakconvexfunc})}{2}
    \ltwos{x_k - x_k^\lambda}^2
    + \stepsize_k^2 B.
  \end{equation}
\end{lemma}
\begin{comment}
\begin{proof}
  Let $\lambda > \E[\weakconvexfunc(\statrv)]$, so that $F(y) +
  \frac{\lambda}{2} \ltwo{y - x}^2$ is strongly convex in $y$.  Then for
  each $k$, we have the bounds
  \begin{align}
    F_\lambda(x_{k+1})
    & = F(x^\lambda_{k+1}) + \frac{\lambda}{2} \ltwos{x^\lambda_{k+1}
      - x_{k+1}}^2
    \le F(x^\lambda_{k}) + \frac{\lambda}{2} \ltwos{x^\lambda_{k}
      - x_{k+1}}^2,
    \label{eqn:shift-lambda-index}
  \end{align}
  by definition of $x^\lambda_{k+1}$. Now, because
  $x_{k+1}$ solves the update~\eqref{eqn:stochastic-prox-point}
  with the model $f_{x_k}$, we have by the standard optimality
  conditions for strongly convex minimization that
  \begin{align*}
    \stepsize_k f_{x_k}(x_{k+1};\statrv_k)
    + \half \ltwo{x_{k+1} - x_k}^2
    + \half \ltwo{y - x_{k+1}}^2
    \le \stepsize_k f_{x_k}(y; \statrv_k) + \half \ltwo{y - x_k}^2
  \end{align*}
  for all $y$. Substituting this inequality into
  Eq.~\eqref{eqn:shift-lambda-index} with the choice $y = x^\lambda_k$, we
  have
  \begin{align}
    F_\lambda(x_{k+1})
    & \le F(x^\lambda_k) +
    \frac{\lambda}{2}\left[
      \ltwos{x^\lambda_k - x_k}^2
      + 2 \stepsize_k\left(f_{x_k}(x^\lambda_k; \statrv_k)
      - f_{x_k}(x_{k+1}; \statrv_k)\right)
      - \ltwo{x_{k+1} - x_k}^2 \right] \nonumber \\
    & = F_\lambda(x_k)
    + \lambda \stepsize_k
    \left[f_{x_k}(x^\lambda_k; \statrv_k)
      - f_{x_k}(x_{k+1}; \statrv_k)
      - \frac{1}{2 \stepsize_k} \ltwo{x_{k+1} - x_k}^2 \right].
    \label{eqn:moreau-little-progress}
  \end{align}
  Because $y \mapsto f_x(y;\statval)$ is convex,
  we have for all $\statval \in \statdomain$ that
  \begin{align*}
    f_{x_k}(x_{k+1};\statval)
    & \ge f_{x_k}(x_k; \statval)
    + \<f'(x_k; \statval), x_{k+1} - x_k\>
    = f(x_k; \statval) + \<f'(x_k; \statval), x_{k+1} - x_k\>.
  \end{align*}
  Thus we have
  \begin{align*}
    \lefteqn{f_{x_k}(x_k^\lambda; \statval)
      - f_{x_k}(x_{k+1}; \statval)} \\
    & \le f(x_k^\lambda; \statval)
    - f(x_k; \statval)
    + \frac{\weakconvexfunc(\statval)}{2} \ltwos{x_k^\lambda - x_k}^2
    + \<f'(x_k;\statval), x_k - x_{k+1}\> \\
    & \le f(x_k^\lambda; \statval)
    - f(x_k; \statval)
    \frac{\weakconvexfunc(\statval)}{2} \ltwos{x_k^\lambda - x_k}^2
    + \frac{\stepsize_k}{2} \ltwo{f'(x_k;\statval)}^2
    + \frac{1}{2 \stepsize_k} \ltwo{x_k - x_{k+1}}^2.
  \end{align*}
  Substituting into inequality~\eqref{eqn:moreau-little-progress} yields
  \begin{equation*}
    F_\lambda(x_{k+1})
    \le F_\lambda(x_k) +
    \lambda \stepsize_k\left[
      f(x_k^\lambda; \statrv_k)
      - f(x_k; \statrv_k)
      + \frac{\weakconvexfunc(\statrv_k)}{2} \ltwos{x_k^\lambda - x_k}^2
      + \frac{\stepsize_k}{2} \ltwo{f'(x_k; \statrv_k)}^2
      \right].
  \end{equation*}
  Taking expectations
  conditional
  $\mc{F}_{k-1}
  = \sigma(\statrv_1, \ldots, \statrv_{k-1})$, noting
  that $x_k \in \mc{F}_{k-1}$ and $x_k^\lambda \in \mc{F}_{k-1}$,
  we have
  \begin{align*}
    \lefteqn{\E\left[f(x^\lambda_k; \statrv_k)
        - f(x_k; \statrv_k) \mid \mc{F}_{k-1}\right]
      + \frac{\E[\weakconvexfunc(\statrv)]}{2} \ltwos{x^\lambda_k - x_k}^2} \\
    & = F(x^\lambda_k) - F(x_k) + \frac{\lambda}{2}
    \ltwos{x^\lambda_k - x_k}^2 - \frac{\lambda -\wb{\weakconvexfunc}}{2}
    \ltwos{x^\lambda_k - x_k}^2
    \le - \frac{\lambda -\wb{\weakconvexfunc}}{2}
    \ltwos{x^\lambda_k - x_k}^2
  \end{align*}
  by definition of $x_k^\lambda$ as the minimizer of $F(y) +
  \frac{\lambda}{2} \ltwos{y - x_k}^2$ over $y$.
  Substituting this above, we obtain
  \begin{equation}
    \label{eqn:semiconvex-progress-with-subgradient}
    \E[F_\lambda(x_{k+1}) \mid \mc{F}_{k-1}]
    \le F_\lambda(x_k)
    - \stepsize_k \frac{\lambda(\lambda - \wb{\weakconvexfunc})}{2}
    \ltwos{x_k^\lambda - x_k}^2
    + \frac{\lambda \stepsize_k^2}{2}
    \E\left[\ltwo{f'(x_k;\statrv_k)}^2 \mid \mc{F}_{k-1}\right].
  \end{equation}
  
  We now consider two cases for
  inequality~\eqref{eqn:semiconvex-progress-with-subgradient}. In the case
  that $f(\cdot; \statval)$ is $\lipobj(\statval)$-Lipschitz, the argument
  is straightforward.  Taking expectations conditional on $\mc{F}_{k-1}$ we
  have $\E[\ltwo{f'(x_k; \statrv_k)}^2 \mid \mc{F}_{k-1}] \le
  \E[\lipobj(\statrv)^2]$.  Substituting this into
  inequality~\eqref{eqn:semiconvex-progress-with-subgradient} immediately
  gives the first inequality~\eqref{eqn:weakly-convex-lipschitz-progress}.
  
  Instead of the assumption that $f(\cdot; \statval)$
  is $\lipobj(\statval)$-Lipschitz, let us now instead assume
  that Assumption~\ref{assumption:growth-subgrads} holds.
  In this case, we require a small lemma.
  \begin{lemma}
    \label{lemma:switch-x-from-growth}
    Let Assumption~\ref{assumption:growth-subgrads} hold.
    For constants $a, b < \infty$, which may depend
    on $\lambda, C_1, C_2$, for all $x \in \mc{X}$ we have
    \begin{equation*}
      F(x) \le a F(x^\lambda) + b.
    \end{equation*}
  \end{lemma}
  \begin{proof}
    We have that $F$ is $\wb{\weakconvexfunc}$-weakly convex, so that
    \begin{equation*}
      F(x) + \<F'(x), x^\lambda - x\>
      \le F(x^\lambda) + \frac{\wb{\weakconvexfunc}}{2}
      \ltwos{x^\lambda - x}^2.
    \end{equation*}
    Using that $\<u, v\> \le \frac{1}{2 \eta} \ltwo{u}^2
    + \frac{\eta}{2} \ltwo{v}^2$ for all $u, v$, the preceding display
    implies
    \begin{equation*}
      F(x) - \frac{1}{2 \eta} \ltwo{F'(x)}^2
      \le F(x^\lambda) + \frac{\wb{\weakconvexfunc} + \eta}{2}
      \ltwos{x^\lambda - x}^2.
    \end{equation*}
    Jensen's inequality
    and Assumption~\ref{assumption:growth-subgrads} imply
    $\ltwo{F'(x)}^2 \le
    \E[\ltwo{f'(x; \statrv)}^2] \le C_1 F(x) + C_2$,
    so
    \begin{equation*}
      \left(1 - \frac{C_1}{2 \eta}\right)F(x)
      \le F(x^\lambda) + \frac{\wb{\weakconvexfunc} + \eta}{2}
      \ltwos{x^\lambda - x}^2 + C_2.
    \end{equation*}
    Finally, by assumption that $x^\lambda$ minimizes
    $F(y) + \frac{\lambda}{2} \ltwo{y - x}^2$ over $y \in \mc{X}$,
    we have
    \begin{equation*}
      \<F'(x^\lambda) + \lambda(x^\lambda - x),
      y - x^\lambda\> \ge 0 ~~ \mbox{for~all~} y \in \mc{X}.
    \end{equation*}
    Setting $y = x$ and rearranging yields
    $\ltwos{x^\lambda - x}^2 \le \lambda^{-1} \<F'(x^\lambda), x - x^\lambda\>$,
    so that Cauchy-Schwarz and Assumption~\ref{assumption:growth-subgrads}
    give
    \begin{equation*}
      \ltwos{x^\lambda - x} \le \lambda^{-1} \ltwos{F'(x^\lambda)}
      \le \lambda^{-1} C_1 F(x^\lambda) + \lambda^{-1} C_2.
    \end{equation*}
    Choosing $\eta > C_1$ gives the result.
  \end{proof}

  Applying Lemma~\ref{lemma:switch-x-from-growth} in
  inequality~\eqref{eqn:semiconvex-progress-with-subgradient},
  we see the constants $a, b$ in Lemma~\ref{lemma:switch-x-from-growth}
  imply the existence of constants $A, B < \infty$
  in inequality~\eqref{eqn:weakly-convex-nonlipschitz-progress},
  completing the proof.
\end{proof}
\end{comment}
The next corollary provides convergence guarantees for our models. To prove this result, we require the almost
supermartingale convergence lemma due to \citet{RobbinsSi71}.
\begin{lemma}[Robbins and Siegmund~\cite{RobbinsSi71}]
	\label{lemma:robbins-siegmund}
	Let $A_k, B_k, C_k, D_k \ge 0$ be non-negative random variables
	adapted to the filtration $\mc{F}_k$. If
	\begin{equation*}
	\E[A_{k + 1} \mid \mc{F}_k] \le (1 + B_k) A_k + C_k
	- D_k,
	\end{equation*}
	then on the event $\{\sum_k B_k < \infty, \sum_k C_k < \infty\}$,
	we have $A_k \cas A_\infty$ for some random variable $A_\infty$ and
	$\sum_k D_k < \infty$.
\end{lemma}
Now we state our main convergence result in this section.
\begin{corollary}
	Let Conditions~\ref{cond:convex-model}--\ref{cond:subgrad-model}
	hold. Let $\hat{x}_k = x_j$ with probability $\frac{\stepsize_j}{\sum_{i=0}^{k} {\stepsize_i}}$ for $0 \le j \le k$. If $f(\cdot;\statval)$ is $\lipobj(\statval)$-Lipschitz, or Assumption~\ref{assumption:growth-subgrads} holds then there exists $C < \infty$ such that
	\begin{equation}
	\E[\ltwo{\hat{x}_k - \hat{x}_k^\lambda}^2 \mid \mc{F}_{k-1}]
	\le \frac{F_{\lambda}(x_0) - \inf_{y \in \mc{X}} F(y) + C \sum_{i=0}^{k}{\stepsize_i^2}}{\frac{\lambda (\lambda - \wb{\weakconvexfunc})}{2} \sum_{i=0}^{k} {\stepsize_i}}.
	\end{equation}	
\end{corollary}
\begin{proof}
	From the definition of $\hat{x}_k$, we have
	\begin{align*}
	\E[\ltwo{\hat{x}_k - \hat{x}_k^\lambda}^2 \mid \mc{F}_{k-1}]
     = \frac{1}{\sum_{i=0}^{k} {\stepsize_i}} \sum_{i=0}^{k}{\stepsize_i \ltwos{x_k - x_k^\lambda}^2} 
	\end{align*}
	If $f$ is $\lipobj(\statval)$-Lipschitz, then we use equation~\eqref{eqn:weakly-convex-lipschitz-progress} to get
	\begin{equation*}
	\E[\ltwo{\hat{x}_k - \hat{x}_k^\lambda}^2 \mid \mc{F}_{k-1}]
	\le \frac{F_{\lambda}(x_0) - \inf_{y \in \mc{X}} F(y) + \frac{\lambda}{2} \E[\lipobj(\statrv)^2] \sum_{i=0}^{k}{\stepsize_i^2}}{\frac{\lambda (\lambda - \wb{\weakconvexfunc})}{2} \sum_{i=0}^{k} {\stepsize_i}}.
	\end{equation*}
	As $\sum_{i=0}^{k}{\stepsize_i^2} < \infty$, the claim follows.
	\noindent
	Now assume Assumption~\ref{assumption:growth-subgrads} holds. 
	We use Lemma~\ref{lemma:robbins-siegmund} with equation~\eqref{eqn:weakly-convex-nonlipschitz-progress} to get that $\sup_{k\in{\N}}{F_\lambda(x_k)} \le F < \infty$. Thus, using this upper bound on $F_\lambda(x_k)$ in~\eqref{eqn:weakly-convex-nonlipschitz-progress} we get
	\begin{equation*}
	\E[F_\lambda(x_{k+1}) \mid \mc{F}_{k-1}]
	\le  F_\lambda(x_k)
	- \stepsize_k \frac{\lambda(\lambda - \wb{\weakconvexfunc})}{2}
	\ltwos{x_k - x_k^\lambda}^2
	+ \stepsize_k^2 (B +  A F).
	\end{equation*}
	The claim now follows by using similar arguments as in the case that $f(\cdot;\statval)$ is Lipschitz.
\end{proof}
	



==> weakly-convex-stability.tex <==
% -*- Mode: latex -*- %

\section{Stability for weakly convex functions}
\label{sec:stability}
The previous section shows that any model satisfying Conditions~{?} will converge to a point close to nearly stationary point; this convergence does not depend on the accuracy of the model. In this section, we start arguing for the importance of choosing accurate models in the update~\eqref{eqn:stochastic-prox-point}. In particular, we prove that certain models enjoy better stability properties, in the sense that their iterates remain bounded. The stability results in this section extend the results presented in Section 3 in~\ref{AD18} to the weakly convex case. 


We begin with our definitions of stability and boundedness which are a relaxed version of the stability definition in~\ref{AD18} (~\ref{AD18} definition 3.1), as it is challenging to prove the same strong stability guarantees in the weakly convex case. In this definition, we let
$\mc{A}$ denote the set of positive stepsize sequences $\{\stepsize_k\}$
with $\sum_k \stepsize_k^2 < \infty$. We call a pair $(\mc{F}, \mc{P})$ a
\emph{collection of problems} if $\mc{P}$ is a collection of probability
measures on a sample space $\statdomain$, and $\mc{F}$ is a collection of
functions $f : \mc{X} \times \statdomain \to \R$. We have the following definition.
\begin{definition}
	\label{definition:weak-stability}
	An algorithm generating
	iterates $x_k$ according to
	the model-based update~\eqref{eqn:stochastic-prox-point}
	is \emph{weakly-stable for the collection} of
	problems $(\mc{F}, \mc{P})$ if for all $f \in \mc{F}$ and $P \in \mc{P}$
	defining $F(x) = \E_P[f(x; \statrv)]$
	and $\mc{X}\opt = \argmin_{x \in \mc{X}} F(x)$, we have
	\begin{subequations}
		\label{eqn:both-stabilities}
		\begin{equation}
		\label{eqn:bounded-expected-distance}
		\sup_{\stepsize \in \mc{A}}
		\sup_{k \in \N} \frac{\E[\dist(x_k, \mc{X}\opt)^2]}{
			\sum_k \stepsize_k} < \infty.
		\end{equation}
		We say the algorithm is bounded if for all stepsize sequences $\{\stepsize_k\} \in \mc{A}$,
		\begin{equation}
		\sup_k \dist(x_k, \mc{X}\opt) < \infty
		~~ \mbox{with~probability~1}.
		\label{eqn:bounded-distance}
		\end{equation}
	\end{subequations}
\end{definition}

The stability definition in~\cite{AD18} require, instead of~\eqref{eqn:bounded-expected-distance}, that
\begin{equation}
\sup_{\stepsize \in \mc{A}}
\sup_{k \in \N} \frac{\E[\dist(x_k, \mc{X}\opt)^2]}{
	\sum_k \stepsize_k^2} < \infty.
\end{equation}
\citet{AD18} prove that accurate models are stable if the functions $f(\cdot; \statrv)$ are convex. Moreover, they present several examples demonstrating that basic models, such as the stochastic subgradient model, are not usually stable. Here, we carry the same task in the weakly convex setting. In particular, we show that accurate models are weakly-stable, in contrast to basic models which usually does not satisfy the weak stability condition~\eqref{eqn:bounded-expected-distance}.
Then, we show that, under certain assumptions, if the models are weakly-stable, then they are also bounded, emphasizing the importance of weak-stability???.
Let us start with several examples, where basic models are not weakly-stable or bounded, in contrast to accurate models that, as we show, are weakly-stable in these settings.

\begin{example}
	weak-stability..(phase retrieval)
\end{example}


\begin{example}
	bounded..(phase retrieval to the power of 4?)
\end{example}

\subsection{Weak stability of accurate models}

\subsection{Boundedness of accurate models}

\newpage
In this section, we prove stability guarantees in the weakly convex case, by proving that the distance of the iterates to the optimal set is polynomially bounded. We begin by proving stability for the full stochastic proximal point method, and then prove similar result for the prox-linear. Finally, by noting that SGM and the truncated model are both special instances of the prox-linear model, we give an additional justification for the better stability of the truncated model. 

\subsection{Stability of the full proximal method}

Here, we provide stability guarantees for the full proximal method in the non convex case by proving upper bounds on the distance to the optimal set. The results in this section rely on two different new assumptions, which are not true for weakly convex functions in general, but hold for popular non convex problems such as phase retrieval~\cite{Fienup78} and matrix completion~\cite{KeshavanMoOh10a}.

First, let us consider the following assumption.
\begin{assumption}
	\label{assm:very-weakly-convex}
	For each $\statval \in \statdomain$, the function $f(\cdot; \statval)$ satisfies
	\begin{equation*}
	\<f'(x;\statval) - f'(y;\statval), x - y \> \geq -C(\statval),
	\end{equation*}
	where $\E[C(\statrv)] < \infty$
\end{assumption}
We prove that the assumption holds true for phase retrieval, and then we prove an upper bound on the distance to the optimal set.
\begin{lemma}
	Let $f(x;(a,b)) = \left| \<a, x\> ^2 - b\right|$. Then, for every $(a, b) \in \R^n \times \R_+$ and $x,y\in \mc{X}$, it holds that
	\begin{equation*}
	\<f'(x;(a, b)) - f'(y;(a, b)), x - y \> \geq -8b.
	\end{equation*}
\end{lemma}
\begin{proof}
	We denote $s_1 =\<\sign(\<a, x\> ^2 - b)$ and $s_2 = \sign(\<a, y\> ^2 - b) $.   Since $\partial f(x; (a, b)) = 2 \sign(\<a, x\> ^2 - b) a^T x a,$ we get 
	\begin{align*}
	z = \<f'(x;(a, b)) - f'(y;(a, b)), x - y \> 
	& = 2 \< s_1 a^T x a - s_2 a^T y a, x - y \> \\
	& = 2 (s_1 a^T x - s_2 a^T y)(a^T x - a^T y) \\
	& = 2 \big(s_1 (a^T x)^2 -(a^T x) (a^T y) (s_1+s_2)  + s_2 (a^T y)^2  \big)
	\end{align*}
	If $s_1 = s_2 =1 $ or $s_1 = -s_2$ then clearly $z \ge 0$. Otherwise, $s_1 = s_2 = -1$, which means that $(a^T x)^2 \le b$ and $(a^T y)^2 \le b$. This implies that $z \ge -8b$. 
\end{proof}

\begin{comment}
\begin{lemma}
	\label{lemma:very-weakly-conv-bound}
	Let $g$ satisfy $	\<g'(x;\statval) - g'(y;\statval), x - y \> \geq -C$ and be subdifferentiable on a closed convex set $\mc{X}$
	and let $\beta > 0$. Then for all $x_0, x_1, y \in \mc{X}$,
	$g'(y) \in \partial g(y)$, and dual
	norms $\norm{\cdot}$ and $\dnorm{\cdot}$,
	\begin{equation*}
	\<g'(x_1), y - x_1\> - C
	\le \<g'(y), y - x_0\>
	+ \frac{1}{2 \beta} \norm{x_1 - x_0}^2
	+ \frac{\beta}{2} \dnorm{g'(y)}^2.
	\end{equation*}
\end{lemma}
\begin{proof}
	By the given assumption, we have
	\begin{align*}
	\<g'(x_1), y - x_1\> - C
	& \le \<g'(y), y - x_1\>
	= \<g'(y), y - x_0\> + \<g'(y), x_0 - x_1\> \\
	& \le \<g'(y), y - x_0\> + \frac{1}{2 \beta} \norm{x_1 - x_0}^2
	+ \frac{\beta}{2} \dnorm{g'(y)}^2,
	\end{align*}
	where the second line uses that $\<a,b\> \le \frac{1}{2 \beta} \norm{a}^2
	+ \frac{\beta}{2} \dnorm{b}^2$ for all $\beta > 0$ and pair
	of dual norms $\norm{\cdot}$ and $\dnorm{\cdot}$.
\end{proof}
\end{comment}

If Assumption~\ref{assm:very-weakly-convex} holds, we can prove a polynomial bound on the expectation of the iterates' distance to the optimal set.
\begin{lemma}
	\label{lemma:stab-weakly-conv_1}
	Let Assumption~\ref{assm:very-weakly-convex} hold. Assume further that $\sqrt{\E [\rho(\statrv_k)^2]} \le \bar{\rho}$. Let $x_k$ be generated by the updates~\eqref{eqn:stochastic-prox-point} using the full proximal \textcolor{red}{model~\eqref{eqn:prox-model}.} Then
	\begin{equation*}
	\E\left[\ltwo{x_{k + 1} - x\opt}^2 \mid \mc{F}_{k-1}\right]
	\le
	\ltwo{x_k - x\opt}^2
	+ \stepsize_k \bar{\rho} (\E [C(\statrv_k)]+\stepsize_k \bar{\rho}  \sigma^2)
	\end{equation*}
\end{lemma}

\begin{comment}
\begin{proof}
	Using the last inequality in Lemma~\ref{lemma:weakly-single-step-progress} and applying Lemma~\ref{lemma:very-weakly-conv-bound} with the choices $x_1 = x_{k + 1}$, $x_0 = x_k$, and
	$y = x\opt$ to find
	\begin{align*}
	\half \ltwo{x_{k + 1} - x\opt}^2 
	& \le \half \ltwo{x_k - x\opt}^2 - \frac 1 {\rho(\statrv_k) + 1/ \stepsize_k} \<g_k, x_{k+1} - x\opt\> - \half \ltwo{x_{k + 1} - x_k}^2 \\
	& \le \half \ltwo{x_k - x\opt}^2 +   \<f'(x\opt; \statrv_k), x\opt - x_k\>
	+ \frac{(\rho(\statrv_k)\stepsize_k)^2}{2}
	\ltwo{f'(x\opt; \statrv_k)}^2 + \rho(\statrv_k)\stepsize_k C(\statrv_k) \\
	%& \le \half \ltwo{x_k - x\opt}^2 +    \<f'(x\opt; \statrv_k), x\opt - x_k\>
	%+ \frac{(\bar{\rho}\stepsize_k)^2}{2}
	%\ltwo{f'(x\opt; \statrv_k)}^2 + \bar{\rho}\stepsize_k C(\statrv_k)
	\end{align*}
	  for all $f'(x\opt; \statrv_k) \in \partial f(x\opt; \statrv_k)$.
	Now, for some $F'(x\opt) \in \partial F(x\opt)$, we have
	$\<F'(x\opt), y - x\opt\> \ge 0$ for all $y \in \mc{X}$.
	We may take $f'(x\opt; \statval) \in \partial f(x\opt; \statval)$
	so that
	$\E[f'(x\opt; \statrv_k)] = F'(x\opt)$ (cf.~\cite{Bertsekas73}), and
	thus, taking expectations with respect to $\mc{F}_{k-1}$, we have
	\begin{equation*}
	\half \E[\ltwo{x_{k + 1} - x\opt}^2 \mid \mc{F}_{k-1}]
	\le \half \ltwo{x_k - x\opt}^2
	+ \frac{(\bar{\rho}\stepsize_k)^2}{2} \E[\ltwo{f'(x\opt; \statrv)}^2]
	+  \<F'(x\opt), x\opt - x_k\> + \stepsize_k \bar{\rho} \E [C(\statrv_k)].
	\end{equation*}
	As $\<F'(x\opt), x\opt - x_k\> \le 0$, we obtain the theorem.
\end{proof}
\end{comment}

Now, we consider a weaker assumption than~\ref{assm:very-weakly-convex} that holds for more functions such as the matrix completion function, where $f(x,y;(i,j)) = \left|\<x_i, y_j\> - M_{i,j}\right|$. 
\begin{assumption}
	\label{assm:very-weakly-convex-modified}
	For each $\statval \in \statdomain$, the function $f(\cdot; \statval)$ satisfies
	\begin{equation*}
	\< f'(x; \statval) , x \> \ge -C(\statval).
	\end{equation*}
\end{assumption}
First, we show different problems where this assumption holds.

\begin{example}
	Phase Retrieval. Let $f(x;(a,b)) = \left|  \<a, x\> ^2 - b\right|$. Then we get
	\begin{align*}
	\< f'(x;(a,b)) , x \>  & = \< 2 \sign( \<a, x\> ^2 - b) a^T x a, x\> \\
	& = 2 \sign(\<a, x\> ^2 - b) (a^T x)^2 \\
	& \ge 
	\begin{cases*}
	0, & \text{if } $\<a, x\> ^2 \ge b$ \\
	-2b,  & \text{otherwise}
	\end{cases*}
	\\ & \ge -2b
	\end{align*}
\end{example}

\begin{example}
	Matrix Completion. Let $f(x,y;(i,j)) = \left|\<x_i, y_j\> - M_{i,j}\right|$. Then we get that
	\begin{equation*}
	f'(x,y;(i,j)) = \sign(\<x_i, y_j\> - M_{i,j}) (y_j, x_i).
	\end{equation*}
	Therefore, we get that
	\begin{align*}
	\< f'(x,y; (i,j)) , (x,y) \>  & = \sign(\<x_i, y_j\> - M_{i,j})  \< (y_j, x_i) , (x_i, y_j) \> \\
	& =  2 \sign(\<x_i, y_j\> - M_{i,j}) \<x_i, y_j\> \\
	& \ge \begin{cases*}
	2M_{i,j}, & \text{if } $\<x_i, y_j\> \ge M_{i,j}$ \\
	-2M_{i,j},  & \text{otherwise}
	\end{cases*}
	\\ & \ge -2 \left| M_{i,j} \right|
	\end{align*}
\end{example}

Now, if Assumption~\ref{assm:very-weakly-convex-modified} holds, we prove that the norm of the iterates is polynomially bounded.
\begin{lemma}
	\label{lemma:stab-weakly-conv_2}
	Let Assumption~\ref{assm:very-weakly-convex-modified} hold.  Let $x_k$ be generated by the updates~\eqref{eqn:stochastic-prox-point} using the full proximal \textcolor{red}{model~\eqref{eqn:prox-model}.} Then
	\begin{equation*}
	\E\left[\ltwo{x_{k + 1}}^2 \mid \mc{F}_{k-1}\right]
	\le
	\ltwo{x_k }^2
	+ 2\stepsize_k \E [C(\statrv_k)].
	\end{equation*}
\end{lemma}
\begin{comment}
\begin{proof}
	Since $x_{k+1} + \stepsize_k g_k^T = x_k$ [\textcolor{red}{fix for the case $\mc{X} \ne R^n$}], we get that
	\begin{align*}
	\ltwo{x_k}^2  & = \ltwo{x_{k+1}}^2 + 2\stepsize_k g_k^T x_{k+1} + \ltwo{\stepsize_k g_k}^2 \\
	& \ge  \ltwo{x_{k+1}}^2 - 2\stepsize_k C(\statrv_k).
	\end{align*}
\end{proof}
\end{comment}

\subsection{Stability of the prox-linear model}
In this section, we consider the composite optimization problem where $f(x; \statrv_k) = h(c(x; \statrv_k); \statrv_k)$ and analyze the prox-linear model~\eqref{eqn:prox-linear-model}.
We prove stability guarantees for this model, stating that the iterates have a polynomially bounded norm. We start by considering two strong assumptions on $c(\cdot)$ and $h(\cdot)$ that are enough to prove stability. Then, we prove similar stability results under weaker assumptions. We choose to start with the strong assumptions as they are easier to understand. 

Let us consider the following assumption on $c(\cdot)$.
\begin{assumption}
	\label{assm:almost_polynomial}
	For each $\statval \in \statdomain$, the functions $c(\cdot; \statval)$ satisfy
	$ \< \nabla c(x; \statval), x \> = \alpha(x; \statval) c(x; \statval)$ where $1 \le \alpha(x;\statval) \le M(\statval)$.
\end{assumption}

If Assumption~\ref{assm:almost_polynomial} holds, then Assumption~\ref{assm:very-weakly-convex-modified} also holds, hence one can prove a polynomial bound for the full proximal method. This is not the case for prox-linear, as we have the counter example $h(y) = y$ and $c(x) = x^2$. However, taking $h(y) = |y|$ and $c(x) = x^2$ still yields the same function $f(x) = x^2$, and now prox-linear is polynomially stable. In this section, we aim to theoretically explain this phenomenon; in particular, we prove that if the function $h(y)$ is convex and $\inf_{y\in R} h(y) > -\infty$, then the prox-linear method is polynomially stable. We will have the following assumption for $h(\cdot)$.
\begin{assumption}
	\label{assm:convex_bounded}
	For each $\statval \in \statdomain$, the functions $h(\cdot; \statval)$ are convex and $\inf_{y\in R} h(y;\statval) \ge m(\statval)$.
\end{assumption}
The following stability guarantee is proved under Assumptions~\ref{assm:almost_polynomial} and ~\ref{assm:convex_bounded}.
\begin{theorem}
	\label{theorem:stab_prox_linear_1}
	Let Assumptions~\ref{assm:almost_polynomial} and ~\ref{assm:convex_bounded} hold. Let $x_k$ be generated by the updates~\eqref{eqn:stochastic-prox-point} using the prox-linear model~\eqref{eqn:prox-linear-model}. Then
	\begin{equation*}
	\E [ \ltwo{x_{k+1}}^2 \mid \mc{F}_{k-1} ] <  \ltwo{x_k}^2   + 2 \stepsize_k \E [ M(\statrv_k) ( m(\statrv_k) - h(0;\statrv_k) ) ] .
	\end{equation*}
\end{theorem}
\begin{comment}
\begin{proof}
	We begin by providing a lower bound for $\<\nabla f_{x_k}(x_{k+1}) , x_{k+1}\>$.
	Denote $\tilde c(x;\statrv_k) = c({x_k};\statrv_k) + \nabla c({x_k}; \statrv_k)^T (x-{x_k})$. One can easily argue that \textcolor{red}{[fix for the case $\mc{X} \ne R^n$]}  
	\begin{equation*}
	x_{k+1} = x_k - \stepsize_k \beta \nabla c(x_k; \statrv_k),
	\end{equation*}
	and therefore
	\begin{equation*}
	\tilde c(x_{k+1}; \statrv_k) = c({x_k}; \statrv_k) - \stepsize_k \beta   \ltwo{\nabla c(x_k); \statrv_k}^2,
	\end{equation*}	
	where $\beta = h'(\tilde c(x_{k+1}; \statrv_k))$. This implies that
	\begin{align*}
	\<\nabla f_{x_k}(x_{k+1}; \statrv_k) , x_{k+1}  \> 
	& =  \left< h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big) \cdot   \nabla c(x_k; \statrv_k), x_k - \stepsize_k \beta \nabla c(x_k; \statrv_k) \right> \\
	& =  h'\big(\tilde c(x_{k+1}; \statrv_k) ; \statrv_k\big) \cdot \big( \< \nabla c(x_k; \statrv_k), x_k \> -\stepsize_k \beta   \ltwo{\nabla c(x_k; \statrv_k)}^2  \big) \\
	& =  h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big) \cdot  \big( \alpha(x_k; \statrv_k) c(x_k; \statrv_k) -\stepsize_k \beta   \ltwo{\nabla c(x_k; \statrv_k)}^2  \big) \\
	& = h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big)  \cdot  \big( c(x_k; \statrv_k) -\stepsize_k \beta   \ltwo{\nabla c(x_k; \statrv_k)}^2  \big) \\
	& + (\alpha(x_k; \statrv_k)-1) \cdot h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big) \cdot c(x_k; \statrv_k) \\
	& = h'\big(\tilde c(x_{k+1}; \statrv_k)\big)  \cdot  \tilde c(x_{k+1}; \statrv_k) 
	 + (\alpha(x_k; \statrv_k)-1) \cdot h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big) \cdot c(x_k; \statrv_k).
	\end{align*}
	Now we prove that each of these two terms is lower bounded. First, since $h(y; \statrv_k)$ is convex, we get that $h'(y; \statrv_k)y \ge h(y; \statrv_k) - h(0; \statrv_k) \ge m(\statrv_k) - h(0; \statrv_k)$, and therefore the first term is lower bounded. Now we proceed to the second term. It is enough to prove that 
	\begin{equation}
	\label{eq_needed0}
	h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big) \cdot \big( \tilde c(x_{k}; \statrv_k) - \tilde c(x_{k+1}; \statrv_k)  \big) \ge 0,
	\end{equation} 
	since this implies that
	\begin{equation*}
	h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big)  \cdot \tilde c(x_{k}; \statrv_k) \\
	\ge 	h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big) \cdot \tilde c(x_{k+1}; \statrv_k ) \\
	\ge m(\statrv_k) - h(0).
	\end{equation*}
	Eq.~\ref{eq_needed0} holds since
	\begin{equation*}
	h'\big(\tilde c(x_{k+1}; \statrv_k); \statrv_k \big) \cdot \big( \tilde c(x_{k}; \statrv_k) - \tilde c(x_{k+1}; \statrv_k)  \big) =  \stepsize_k h'(\tilde c(x_{k+1}; \statrv_k); \statrv_k)^2   \ltwo{\nabla c(x_k; \statrv_k)}^2 \ge 0.
	\end{equation*}
	To conclude, we proved that 
	\begin{equation*}
	\<\nabla f_{x_k}(x_{k+1}) , x_{k+1}  \> \ge - M(\statrv_k) ( m(\statrv_k) - h(0) ).
	\end{equation*}
	Now, the standard optimality conditions for convex functions implies that
	\begin{align*}
	\ltwo{x_k}^2 \ge  
	  \ltwo{x_{k+1}}^2 
	  + 2 \stepsize_k \<\nabla f_{x_k}(x_{k+1}) , x_{k+1}\> 
	  +  \ltwo{x_{k+1} - x_{k}}^2,
	\end{align*}
	hence the claim holds.
\end{proof}
\end{comment}

The previous theorem implies the following bounds for phase retrieval and matrix completion.

\begin{example}
	Phase Retrieval. Let $f(x;(a,b)) = \left|  \<a, x\>^2 - b\right|$. Thus, we have $h(y;(a,b)) = \left| y - b\right|$, and $c(x;(a,b)) = \<a, x\>^2$. Theorem~\ref{theorem:stab_prox_linear_1} implies
	\begin{equation*}
	\E [ \ltwo{x_{k+1}}^2 \mid \mc{F}_{k-1} ] <  \ltwo{x_k}^2  + 4 \stepsize_k \E [b] .
	\end{equation*}
\end{example}

\begin{example}
	Matrix Completion. Let $f(x,y;(i,j)) = \left|\<x_i, y_j\> - M_{i,j}\right|$. Thus, we have $h(z;(i,j)) = \left|z - M_{i,j} \right|$, and $c(x,y;(i,j)) = \<x_i, y_j\>$. Theorem~\ref{theorem:stab_prox_linear_1} implies
	\begin{equation*}
	\E [ \ltwo{x_{k+1}}^2 \mid \mc{F}_{k-1} ] <  \ltwo{x_k}^2   + 4 \stepsize_k \E [\left| M_{i,j} \right|] .
	\end{equation*}
\end{example}

We note that Assumption~\ref{assm:almost_polynomial} is satisfied by many other functions. First, it is obvious that $c(x) = a^T x$ and $c(x) = x^T A x$ satisfy the assumption. The following lemma proposes several methods to construct new functions that also satisfy it.


\begin{lemma}
	Let $c_1(x)$ and $c_2(x)$ be such that $\nabla c_i(x)^T x = \alpha_i(x) c_i(x)$ where $1 \leq \alpha_i(x) \leq M_i$. Then the following holds.
	
	\begin{enumerate}
		\item For $\beta \in \R$, $c(x) = \beta \cdot c_1(x)$ satisfies $\nabla c(x)^T x = \alpha(x) c(x)$ where $1 \leq \alpha(x) \leq M_1 $.
		\item $c(x) = c_1(x) \cdot c_2(x)$ satisfies $\nabla c(x)^T x = \alpha(x) c(x)$ where $1 \leq \alpha(x) \leq M_1 + M_2$.
		\item $c(x) = c_1\big( c_2(x) \big)$ satisfies $\nabla c(x)^T x = \alpha(x) c(x)$ where $1 \leq \alpha(x) \leq M_1 \cdot M_2$.
		\item $c(x) = \left| c_1(x) \right| $ satisfies $\nabla c(x)^T x = \alpha(x) c(x)$ where $1 \leq \alpha(x) \leq M_1$.
		\item If $c_1(x) \ge 0$ and $c_2(x) \ge 0$, then $c(x) = c_1(x) + c_2(x)$ satisfies $\nabla c(x)^T x = \alpha(x) c(x)$ where $1 \leq \alpha(x) \leq \max (M_1, M_2)$.
		\item For $n \ge 1$, $c(x) = \big( c_1(x) \big)^n $ satisfies $\nabla c(x)^T x = \alpha(x) c(x)$ where $1 \leq \alpha(x) \leq n \cdot M_1$.
		\item $c(x) = \left| c_1(x) \right| + \left| c_2(x) \right|$ satisfies $\nabla c(x)^T x = \alpha(x) c(x)$ where $1 \leq \alpha(x) \leq \max (M_1, M_2)$.	
	\end{enumerate}
	
\end{lemma}

Now, we give weaker versions of the previous assumptions on $c(x)$ and $h(y)$.
\begin{assumption}
	\label{assm:almost_polynomial_general}
	For each $\statval \in \statdomain$, the functions $c(\cdot; \statval)$ satisfy $\left| \< \nabla c(x;\statval), x \> - \alpha(x;\statval) c(x;\statval) \right| \le C $ where $1 \leq \alpha(x;\statval) \le M(\statval) $.
\end{assumption}

\begin{assumption}
	\label{assm:convex_region_bounded}
	For each $\statval \in \statdomain$, the functions $h(\cdot; \statval)$ are convex, $\inf_{y\in R} h(y;\statval) \ge m(\statval)$, and $\max_{y: \ltwo{y} \le C} h(y;\statval) \le R(\statval)$.
\end{assumption}
Then, we can prove the following theorem.
\begin{theorem}
	\label{theorem:stab_prox_linear_2}
	Let Assumptions~\ref{assm:almost_polynomial_general} and ~\ref{assm:convex_region_bounded} hold. Let $x_k$ be generated by the updates~\eqref{eqn:stochastic-prox-point} using the prox-linear model~\eqref{eqn:prox-linear-model}. Then
	\begin{equation*}
	\E [ \ltwo{x_{k+1}}^2 \mid \mc{F}_{k-1} ] <  \ltwo{x_k}^2  + 2 \stepsize_k \E [ M(\statrv_k) ( m(\statrv_k) - R(\statrv_k) ] .
	\end{equation*}
\end{theorem}

Theorem~\ref{theorem:stab_prox_linear_2} reveals an interesting disparity between the stochastic subgradient method and the truncated model~\eqref{eqn:trunc-model}. Note that given a function $f(x; \statrv_k)$, both methods can be seen as special instances of prox-linear; the former uses $c(x; \statrv_k) = f(x; \statrv_k)$ and $h(y; \statrv_k) = y$, whereas the later uses $c(x; \statrv_k) = f(x; \statrv_k)$ and $h(y; \statrv_k) = \max\{y, \inf_{x\in \mc{X}} f(x\opt; \statrv_k) \}$. Therefore, Theorem~\ref{theorem:stab_prox_linear_2}, under certain conditions on $f(x;\statrv_k)$, implies polynomial stability only for the truncated model, as the assumptions on $h(y)$ are not satisfied for the stochastic subgradient method.
	
Consider, for example, the linear regression setting $f(x; (a,b)) = (a^T x - b)^2$ or the phase retrieval setting $f(x; (a,b)) = \left| \< a,x \>^2 - b \right| $. It is not hard to show that $f(x; (a,b))$ satisfies Assumption~\ref{assm:almost_polynomial_general} in both settings, and hence we have polynomial stability for the truncated model (though, we have earlier proved a stronger sense of stability for linear regression). In contrast, the distance of SGM iterates from
the optimal set can exponentially grow in these problems.





